Rethinking Time Encoding via Learnable Transformation Functions

Effectively modeling time information and incorporating it into applications or models involving chronologically occurring events is crucial. Real-world scenarios often involve diverse and complex time patterns, which pose significant challenges for time encoding methods. While previous methods focus on capturing time patterns, many rely on specific inductive biases, such as using trigonometric functions to model periodicity. This narrow focus on single-pattern modeling makes them less effective in handling the diversity and complexities of real-world time patterns. In this paper, we investigate to improve the existing commonly used time encoding methods and introduce Learnable Transformation-based Generalized Time Encoding (LeTE). We propose using deep function learning techniques to parameterize non-linear transformations in time encoding, making them learnable and capable of modeling generalized time patterns, including diverse and complex temporal dynamics. By enabling learnable transformations, LeTE encompasses previous methods as specific cases and allows seamless integration into a wide range of tasks. Through extensive experiments across diverse domains, we demonstrate the versatility and effectiveness of LeTE.

==> alg_fourier.tex <==
\begin{algorithm}[htb]
\caption{NaiveFourierKANLayer: Initialization and Forward Pass}
\label{alg:NaiveFourierKANLayer}
\begin{algorithmic}[1]

\STATE \textbf{Input:} Timestamp or time difference $t$
\STATE \textbf{Output:} Time embedding $\textbf{t2v+}$
\STATE \textbf{Hyperparameter:} The time encoding dimension $D$, the number of Fourier frequencies index $K$
\STATE \textbf{Initialization:} Initialize learnable weights $\mathbf{W}^{(\text{proj.)}}$, $\mathbf{W}^{(\cos)}$, $\mathbf{W}^{(\sin)}$, $\mathbf{b}^{(\text{proj.)}}$, $\mathbf{b}^{(\text{fourier)}}$.

\STATE Calculate projected time using linear transformation: $ \mathbf{t_{\text{proj.}}} = \mathbf{W}^{(\text{proj.)}}t + \mathbf{b}^{(\text{proj.)}} \in \mathbb{R}^d$
\STATE Calculate Fourier-based \ours: $\textbf{t2v+} = \sum_{i=1}^{D} \sum_{d=1}^{k} \bigl( \mathbf{W}^{(\cos)} \cos(k \mathbf{t_{\text{proj.}}}_i) + \mathbf{W}^{(\sin)} \sin(k \mathbf{t_{\text{proj.}}}_i) \bigr) + \mathbf{b}^{(\text{fourier)}}$




\STATE \textbf{return} $\textbf{t2v+}$

\end{algorithmic}
\end{algorithm}

==> fig_entropy_intro.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figs/entropy_ts.pdf}
\caption{Density plot of spectral entropy for dynamic graph datasets. A lower entropy value indicates periodicity, while a higher entropy value suggests randomness.}
\label{fig:entropy_intro}
% \vspace{-20pt}
\end{figure}

